DiCOVA Challenge: Dataset, task, and baseline system for COVID-19 diagnosis using acoustics

The DiCOVA challenge aims at accelerating research in diagnosing COVID-19 using acoustics (DiCOVA), a topic at the intersection of speech and audio processing, respiratory health diagnosis, and machine learning. This challenge is an open call for researchers to analyze a dataset of sound recordings collected from COVID-19 infected and non-COVID-19 individuals for a two-class classification. These recordings were collected via crowdsourcing from multiple countries, through a website application. The challenge features two tracks, one focusing on cough sounds, and the other on using a collection of breath, sustained vowel phonation, and number counting speech recordings. In this paper, we introduce the challenge and provide a detailed description of the task, and present a baseline system for the task.

==> plot_test_roc_conf_matrices.tex <==

\begin{tikzpicture}
% ----- row 1: put the images
\node[inner sep=0pt,anchor=center] (main_fig) at (4,16) % {x,y} from left corner in an imagined grid
{\includegraphics[width=6cm,height=5.5cm]{figures/IS2021_test_ROCs_fit.pdf}};

\node[inner sep=0pt,anchor=center] (main_fig) at (4,11.5) % {x,y} from left corner in an imagined grid
{\includegraphics[width=8cm,height=2.75cm]{figures/IS2021_test_confusion_matrices_fit.pdf}};

% % ----- put axis labels
% \node[font=\fontsize{8}{6}\selectfont,rotate=0,anchor=center] at (2,12.5) (l1) {Full Test set};
% \node[font=\fontsize{8}{6}\selectfont,rotate=0,anchor=center] at (8,12.5) (l1) {Gender-split Test set};
% \node[font=\fontsize{8}{6}\selectfont,rotate=0,anchor=center] at (14,12.5) (l1) {Age-split Test set};

\end{tikzpicture}


==> table_entire_baseline_system.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{@{}cllrr@{}}
\toprule
\textbf{Track} & \textbf{Sound} & \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Performance \\ (AUC\%)\end{tabular}}} \\ \cmidrule(l){4-5} 
 &  &  & Val. (std. err) & Test \\ \midrule
\textbf{} & \textbf{} & LR & 66.95 ($\pm$ 1.74) & 61.97 \\
1 & Cough & MLP & 68.54 ($\pm$ 1.65) & \textbf{69.85} \\
 &  & RF & 70.69 ($\pm$ 1.39) & 67.45 \\ \midrule
\textbf{} & \textbf{} & LR & 60.95 ($\pm$ 2.17) & 60.94 \\
 & Breathing & MLP & 72.47 ($\pm$ 1.96) & 71.52 \\
 &  & RF & 75.17 ($\pm$ 1.23) & \textbf{76.85} \\ \cmidrule(l){2-5} 
 & \textbf{} & LR & 71.48 ($\pm$ 0.55) & 67.71 \\
2 & Vowel {[}i{]} & MLP & 70.39 ($\pm$ 1.84) & 73.19 \\
 &  & RF & 69.73 ($\pm$ 1.93) & \textbf{75.47} \\ \cmidrule(l){2-5} 
 & \textbf{} & LR & 68.93 ($\pm$ 1.09) & 61.22 \\
 & Speech & MLP & 73.57 ($\pm$ 0.71) & 61.13 \\
 &  & RF & 69.61 ($\pm$ 1.56) & \textbf{65.27} \\ \bottomrule
\end{tabular}
\caption{The baseline system performance on Track-1 and Track-2 datasets.}
\label{tab:baseline_aucs_old}
\end{table}

